PhD Thesis on Code Modulated Interferometric Imaging System using Phased Arrays

This work presents techniques which can allow low-cost phased-array receivers to be reconfigured as interferometric imagers and thereby reducing cost. Since traditional phased arrays power combine incoming signals prior to digitization, orthogonal code-modulation is applied to each incoming signal using phase shifters within each front-end. These code-modulated signals can then be combined and processed coherently through a shared hardware path. Visibility functions can be recovered through squaring and code-demultiplexing operations. The proposed system modulates incoming signals but demodulates desired correlations. Firstly, we present the operation of the system, a validation of its operation using behavioral models of a traditional phased array and a benchmarking of the code-modulated interferometer against traditional interferometer using simulation results and sensitivity analysis. Secondly, we present a simple CMI system operating in the license-free 60-GHz band using a four-element phased-array receiver. The four-element phased array is thinned to obtain a 13-pixel image and the system is demonstrated through a point-source detected at different locations. Finally, the operation and capabilities of code-modulated interferometry (CMI) are demonstrated at 10-GHz using commercially-available phased arrays. A 33-pixel, eight-element prototype is created using two commercially-available ADAR1000 phased-array receivers from Analog Devices Inc. The chips are connected at board level to a patch antenna array. The 33-pixel camera is demonstrated in hardware for point-source detection. Further to demonstrate the scalability of the concept, a 16-element, 169-pixels CMI imaging system is presented at 10-GHz using the four of the same commercially-available phased arrays from ADI. Two active point sources are imaged simultaneously to present the resolution of the system.

==> Chapter-5/Chapter-5.tex <==
\chapter{Scalable imaging system using radio or radars}
\label{chap-five}

\section{Overview} \label{t3-background}

 The outcomes of this thrust will be a detailed study of the feasibility of the approach, including imaging performance estimates (resolution, sensitivity, and field of view), power consumption, heat removal requirements, and cost for n-element 2-D code-modulated interferometric imaging system.

\subsection{Technical Approach} \label{t3-technical}
As part of Objective 1, there are four primary hardware options under consideration for developing the 2-D prototype for the imaging application, as follows: 
\begin{enumerate}
  \item COTS 60 GHz arrays: the radio transceiver arrays which have been released include IBM's 60GHz transceivers chip and 60GHz WiHD Transmitter and Receiver Module Pair by Lattice Semiconductor (DVDO Air3C pro).
  \item In-house 60GHz phased array as discussed in section \ref{t2} which are then tiled to create a larger system. Outputs must be power combined at 60 GHz. 
   \item In-house 28GHz phased array transceivers developed under a parallel program, which can then be tiled to create a larger system. Outputs can be power combined at baseband, as the receiver includes a downconversion mixer.
   \item COTS or custom NCSU vehicular radar transceivers at 76-81 GHz. The latter radar transceivers have been designed by our research group at NC State in collaboration with a commercial partner  Asahi Kasei Microdevices (AKM) using low-cost SiGe technology.  
\end{enumerate}

One of the above hardware will be selected based on the availability and ease of re-configuration. There are challenges and benefits associated with each of the options. The advantage with using a commercially available radio is the packaging with antennas. For the commercially available 60-GHz transceiver/radio, we will need to obtain permissions related to the IP and further information will be needed about the control signals to operate the chip, especially for the code-modulation in the phase-shifters. Up to now, when contacting companies having 60GHz hardware, they have not been willing to work with NCSU to provide either evaluation samples or samples which can be purchased. The advantages of using NCSU custom ICs is that we have easy access to the chips and complete understanding of the parts. The disadvantages relate to the need to develop custom packages and antennas.

As part of the preliminary work, code-modulated interferometry has been developed and modeled for radios and due to fundamental difference in the circuitry of radar, more research will be required to use the vehicular radars. The advantage is that the radar chips feature high output power in the transmitter, high dynamic range in the receiver, and low phase noise in the oscillator and appear well suited for the application of active imaging. The easiest option could be using the in-house 60GHz phased array that would have been already used for the one-D imaging. The difference will be in the packaging, since the output signal will also need to be RF for this case. The RF output of multiple chips will have to be power combined, and square on board or an external power detector will have to be used. Apart from the differences in hardware, the application of code-modulated interferometry, data acquisition and image processing remains similar in either of the four approaches. 

I propose a 12 element imaging system prototype, for example, by using three of the 4-element 60GHz phased array or transceiver. The antennas can be arranged in either "Y" or "T" configurations with each hand consisting of 4 elements. "Y" provides lesser number of redundant baselines and therefore more number of pixels whereas the "T" structure offers ease of design. It is to be noted that the polarization of the antennas has be considered while designing the system. For tiling the same 1-D array thrice to form  a "T", antennas can be designed with circular polarization though with a penalty of $3 dBi$ lower antenna gain. The measurement set up and data acquisition techniques remain same as section \ref{t2}.

==> Makefile <==
CHAPTERS=Chapter-*/Chapter-*.tex  Appendix-*/Appendix-*.tex
NAME=YourName-thesis
AUX=$(NAME).aux front.aux Chapter-*/*.aux Appendix-*/*.aux optional.aux
INTERMEDIATES=$(NAME).bbl $(NAME).blg $(NAME).lof $(NAME).lot \
              $(NAME).log $(NAME).toc 

$(NAME).pdf : $(NAME).tex $(NAME).bib front.tex $(CHAPTERS) ncsuthesis.cls optional.tex
	pdflatex $(NAME)
	bibtex $(NAME)
	pdflatex $(NAME)
	pdflatex $(NAME)

clean :
	rm $(AUX) $(INTERMEDIATES)



